ReLeTA: Reinforcement Learning for Thermal-Aware Task Allocation on Multicore

In this paper, we propose \textit{ReLeTA}: Reinforcement Learning based Task Allocation for temperature minimization. We design a new reward function and use a new state model to facilitate optimization of reinforcement learning algorithm. By means of the new reward function and state model, \releta is able to effectively reduce the system peak temperature without compromising the application performance. We implement and evaluate \releta on a real platform in comparison with the state-of-the-art approaches. Experimental results show \releta can reduce the average peak temperature by 4 $^{\circ}$C and the maximum difference is up to 13 $^{\circ}$C.

==> ProposedApproach.tex <==
\section{\textbf{PROPOSED APPROACH}}
\begin{figure}[htbp]
\centering
\includegraphics[width=\columnwidth]{pictures/flow_chat.png}%fig1
\caption{Proposed system level approach.}
\label{system_level_approach}
\end{figure}

The  Figure \ref{system_level_approach} is our thermal management method based on reinforcement learning dynamic task mapping. Our method is mainly divided into three parts: algorithm control layer, operating system and hardware layer. Our algorithm implements good interaction between the operating system and the hardware layer and achieves a reasonable task mapping.

In order to ensure performance, our method will set the Frequency adjustment mode to ondemand mode when it starts running, so that the system will dynamically adjust the frequency of the core according to the load condition of each core to achieve the effect of reducing the temperature while ensuring system performance.
Whenever a task enters the system, our algorithm reads the frequency and utilization of each core from the hardware as our system state through the operating system, and calculates the q value of each task mapping
the way in the current state through the DQN algorithm. Select the appropriate core and map the task to the corresponding core. When the task starts running, it reads the temperature status of all the cores from the sensor to calculate the reward and timely feedback on the action of the agent. Our method uses the dqn algorithm in reinforcement learning because our state space is continuous and Q-learning is not suitable for our model (the q of all actions of all state is stored in the form of a table, continuous state space will bring huge memory overhead). Therefore, the update problem of Q-Table is turned into a function fitting problem, and similar states get similar output actions. DQN combines deep learning models with reinforcement learning to successfully learn control strategies directly from high-dimensional input.

The q-earning q value is updated in the formula (1)

\begin{equation}
    \begin{split}
&Q(S_i,A_i)\leftarrow Q(S_i,A_i)+\alpha (R_{i+1}+\lambda maxQ(S_{i+1},a)-
&Q(S_i,A_i))
    \end{split}
\end{equation}


Q-learning stores the Q value of the corresponding action into the Q table, while deep-q-learning replaces the Q table with the neural network to approximate the Q value.
Dqn:
\begin{equation}
    \begin{split}
&Q(s,a)= w_1s+w_2a+...+w_na+b 
    \end{split}
\end{equation}

\begin{equation}
    \begin{split}
&Q(s,a)= f(s,a,w) 
    \end{split}
\end{equation}

Dqn approximates Q value by function. The loss function is expressed as:

\begin{equation}
    \begin{split}
L(w)=E[(r+\gamma maxQ(s~',a~',w)-Q(s,a,w))^2]
    \end{split}
\end{equation}

The parameter W is updated by gradient descent of loss (L (w)).



The following is a detailed definition of the elements in our reinforcement learning method:

In our method, we read out the current frequency and utilization of all logic cores from the system as the current state. When assigning tasks using reinforcement learning, we use the vector of current frequency and utilization as the current state of the environment.

$ S= \{F_1, F_2 ... F_n, U_1, U_2,... U_n\} $

After each acquisition of the system state, our method assigns tasks to the core that it considers most appropriate, that is, the action space in reinforcement learning is defined as:

$Action=\{1, 2, 3 ... n\}$

For reward settings, we initially chose the negative average temperature $(-meanTem) $ of the task from the point of view of lowering the overall temperature. Experiments show that the maximum temperature of the system fluctuates greatly in this case, because in many cases, even when agents take different actions, the temperature of individual cores varies greatly. However, the average temperature does not differ much or even remain unchanged, which leads to reward not playing a good role in guiding agents. In addition, we also refer to reward $(threshold temperature - current maximum temperature) $ in the comparative paper 1. It has two problems: 1. In many cases, the maximum temperature is basically equal, resulting in frequent occurrence. The rewards of different actions are basically the same, which is not conducive to agent learning. 2. In many cases, the core with the highest temperature is not necessarily the core with which the program is running, which leads to the lack of correlation between actions and returns (many actions have no direct impact on returns). In combination with the above, we set up a new reward. The following is the definition of reward in our method:

\begin{equation}
Reward_t=\left\{
\begin{aligned}
& 10&   meanTem_{t-1} > actionTem_t \\
& 0 &   meanTem_{t-1} = actionTem_t \\
& 10 &  meanTem_{t-1} < actionTem_t
\end{aligned}
\end{equation}
After each task assignment, we will read all sensors' temperature values and calculate their mean value as $meantem_{t-1}$. When the next task assignment is completed, we will read the temperature value $actionTem_t$ of the running core of the task.
If $actionTem_t>meantem{t-1}$, we will give the agent a reward of $-10$. If $actionTem_t = meanTem_{t-1}$, we will give the agent a prize. The excitation value is 0. If $actionTem_t<meanTem_{t-1}$, we give the agent a reward of 10.
The pseudo-code of our approach :


\begin{algorithm}[H]  
\caption{ Reinforcement Learning for Thermal-Aware Task Allocation on Multicore Systems} 
\label{alg:Framwork}  

\State Initialize reply memory D to capacity N;  
\State Initialize action-value function with random weights   $\theta$;
\State Initialize target action-value function Q with weights 
$\theta\overline=\theta$; 
\State For $episode=1$ , M do
\State  \quad get frequency and utilization of all core as $x_1$ 
\State  \quad Initialize sequence $s_1=\{x_1\}$ and preprocessed
\State  \quad $\phi_1=\phi(s_1)$;
\State \quad sequence $\phi_1$;
\State \quad For $t=1$ ,T do;
\State \qquad Get temperature of all cores through sensor \State \qquad and compute average temperature 
\State \qquad$meanTem_{t-1}$;
\State \qquad With probability $ \epsilon $ select a random core  $a_t$;
\State \qquad otherwise select  $a_t=argmax_a Q(\phi(s_t),a;\theta)$;
\State \qquad set application affinity as $a_t$;
\State \qquad get frequency and utilization of all core as \State \qquad$x_{t+1}$  and get average temperature
\State \qquad $meanTem_t$ and  temperature of running task 
\State \qquad $actionTem_t$;
\State \qquad compute $r_t$ through formula (5);
\State \qquad Set $S_{t+1}=s_t,a_t,x_{t+1}$ and   preprocess 
\State \qquad$\phi_{t+1}=\phi(s_{t+1})$;
\State \qquad Store transition $(\phi_t,a_t,r_t,\phi_{t+1})$;
\State \qquad Sample random minibatch of transitions 
\State \qquad$(\phi_j,a_j,r_ j,\phi_{j+1})$ from D;

\State \qquad  $ Set\ y_j=\left\{
\begin{aligned}
\qquad \qquad r_j  \qquad \qquad  for\ terminal\  \phi_{j+1}\\
r_j+ \gamma max_a Q^{*} (\phi_{j+1},a^{'};\theta) \quad otherwise
\end{aligned}
$;
\State \qquad Perform a gradient descent step on 
\State \qquad$(y_j-q(\phi_j,a_j;\theta))^2$ with respect to the 
\State \qquad network parameters $\theta$;
\State \qquad Every C steps reset $\varrho=\varrho$
\State \qquad End For
\State \quad End For
\end{algorithm}  

